A Characterization of Semiglobal, Practical, Asymptotic Stability for Gain-Parametrized Systems

We consider a general class of nonlinear, constrained, discrete-time systems whose dynamics are parametrized by a set of gains. We define the semiglobal, practical, asymptotic stability (SPAS) of compact sets for this class of systems, and we provide a Lyapunov characterization of such sets. A set A that is SPAS with respect to a given system need not be an attractor for that system. Relative to existing characterizations of similar qualitative behaviors, our SPAS theorem does not require the existence of an asymptotically stable attractor associated to a nominal counterpart of the given dynamics.

==> submitted files/MyPreamble.tex <==

% PACKAGES:
\usepackage{graphics} % for pdf, bitmapped graphics files
\usepackage{epsfig} % for postscript graphics files
\usepackage{mathptmx} % assumes new font selection scheme installed
\usepackage{times} % assumes new font selection scheme installed
\usepackage{amsmath} % assumes amsmath package installed
\usepackage{amssymb}  % assumes amsmath package installed
\usepackage{psfrag}
\usepackage{textcomp}
\usepackage{amsthm}
\usepackage{setspace}
\usepackage{hyperref}
\usepackage{wasysym}
\usepackage{latexsym}
\usepackage{xfrac}
\usepackage{relsize}
\usepackage{pmat}
\usepackage{url}
\usepackage{comment}
\usepackage{pdfsync}

\usepackage[cal=cm]{mathalfa} %this is to get the proper caligraphic font \mathcal and \mathbb (google mathalfa for documentation on how to use)




%\usepackage[margin=1in]{geometry}



%\usepackage[latin1]{inputenc}

% MY COMMANDS
\newcommand{\dt}{\frac{d}{dt}}
\newcommand{\pd}[2]{\frac{\partial #1}{\partial #2}}
\newcommand{\tpd}[2]{\tfrac{\partial #1}{\partial #2}}
\newcommand{\aHalf}{\frac{1}{2}}
\newcommand{\aFourth}{\frac{1}{4}}
\DeclareMathOperator{\blkdiag}{blkdiag}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\spn}{span}
\DeclareMathOperator*{\argmin}{arg\;min}
\DeclareMathOperator{\co}{co}
\newcommand{\del}{\nabla}
\newcommand{\vs}{V_{\Sigma}}
\newcommand{\vo}{V_{\mathcal{O}}}
\newcommand{\dvo}{\Delta V_{\mathcal{O}}}
\newcommand{\dv}{\Delta v^k}
\newcommand{\ol}{\Omega_{\mathit{l}}}
\newcommand{\dvoh}{\Delta V_{\hat{\mathcal{O}}}}
\newcommand{\oh}{\hat{\mathcal{O}}}
\newcommand{\omo}{\Omega_{\mathcal{O}}}
\newcommand{\oms}{\Omega_{\Sigma}}
\newcommand{\omz}{\Omega_z}
\newcommand{\dis}{|y-y^*|}
\newcommand{\dist}{\|y-\mathbf{P}_{X^*}(y)\|}
\newcommand{\1}{\mathbf{1}}
\newcommand{\0}{\mathbf{0}}
\newcommand{\delxi}{\del_{\!\!x_i}}
\newcommand{\sumiv}{\sum_{i\in\mathcal{V}}}
\newcommand{\N}{\mathcal{N}}
\newcommand{\Iota}[1]{\mathlarger{\iota}_{#1}\!}
\newcommand{\lst}[1]{\langle {#1} \rangle\!}
\newcommand{\lsti}[2]{\langle {#1} \rangle\!_{{#2}}^{-1}}
\newcommand{\eg}{{e.g., }}
\newcommand{\ie}{{\it i.e., }}
\newcommand{\st}{\:|\:}
\newcommand{\Pxi}{\mathbf{P}_{X_i}}
\newcommand{\PXi}{\mathbf{P}_{\Xi}}
\newcommand{\Pxhat}{\mathbf{P}_{\hat{X}}}
\newcommand{\Pxst}{\mathbf{P}_{X^*}}
\newcommand{\Pgo}{\mathbf{P}_{\Gamma_0}}
\newcommand{\Pc}{\mathbf{P}_{S}}
\newcommand{\Pa}{\mathbf{P}_{\!\!\mathcal{A}}}
\newcommand{\AIn}{(A\otimes I_n)}
\newcommand{\MIn}{(M\otimes I_n)}
\newcommand{\onetin}{(\mathbf{1}_N^T\otimes I_n)}
\newcommand{\Vo}{V_{\mathcal{O}}}
\newcommand{\Vc}{V_{\mathcal{C}}}
\newcommand{\Ap}{\mathcal{A}^{\bot}}
\newcommand{\Bxst}[1]{\bar{B}_{#1}(X^*)}
\newcommand{\Bgo}[1]{\bar{B}_{#1}(\Gamma_0)}
\newcommand{\Bsqy}{ \bar{B}^n_{\!\!\!\!\sqrt{\sfrac{\delta}{2}}}(X^*)}
\newcommand{\Bsqz}{ \bar{B}^{Nn}_{\!\!\!\sqrt{\sfrac{\delta}{2}}}(\{\0\})}


% MATH OPERATORS
%\DeclareMathOperator{\blkdiag}{blkdiag}
\DeclareMathOperator{\dg}{diag}
\DeclareMathOperator{\setspan}{span}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\Int}{Int}
\DeclareMathOperator{\tr}{tr}

% THEOREM STYLES
 \theoremstyle{remark} %makes defs etc not italic. Must use with amsthm package
\newtheorem{assump}{A\!\!}[section]
\newenvironment{assumpPrime}[1]
  {\renewcommand{\theassump}{\ref{#1}$'$}%
   \addtocounter{assump}{-1}%
   \begin{assump}}
  {\end{assump}}
\newtheorem{lemma}{Lemma}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{claim}{Claim}[section]
\newtheorem{example}{Example}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{defn}{Definition}[section]
\newtheorem{rem}{Remark}[section]
\newtheorem{alg}{Algorithm}[section]
\newtheorem{constr}{Construction}[section]


